Symmetry fractionalization, mixed-anomalies and dualities in quantum spin models with generalized symmetries

We investigate the gauging of higher-form finite Abelian symmetries and their sub-groups in quantum spin models in spatial dimensions $d=2$ and 3. Doing so, we naturally uncover gauged models with dual higher-group symmetries and potential mixed 't Hooft anomalies. We demonstrate that the mixed anomalies manifest as the symmetry fractionalization of higher-form symmetries participating in the mixed anomaly. Gauging is realized as an isomorphism or duality between the bond algebras that generate the space of quantum spin models with the dual generalized symmetry structures. We explore the mapping of gapped phases under such gauging related dualities for 0-form and 1-form symmetries in spatial dimension $d=2$ and 3. In $d=2$, these include several non-trivial dualities between short-range entangled gapped phases with 0-form symmetries and 0-form symmetry enriched Higgs and (twisted) deconfined phases of the gauged theory with possible symmetry fractionalizations. Such dualities also imply strong constraints on several unconventional, i.e., deconfined or topological transitions. In $d=3$, among others, we find, dualities between topological orders via gauging of 1-form symmetries. Hamiltonians self-dual under gauging of 1-form symmetries host emergent non-invertible symmetries, realizing higher-categorical generalizations of the Tambara-Yamagami fusion category.

==> Appendices/2+1d_DW_theory.tex <==
Dijkgraaf-witten theories \cite{Dijkgraaf:1989pz} with the gauge group $\mbb Z_n$ are classified by $H^{3}(\mbb Z_n,\ms U(1))\cong \mbb Z_n$. Given an element ${\rm p} \in \mbb Z_{n}$, one may define a topological action as 
\begin{equation}
    S=\frac{i n}{2\pi}\int \widehat{a}\wedge {\rm{d}}a+\frac{i\rm p}{2\pi}\int a\wedge {\rm{d}}a+\frac{i}{2\pi}\int \left[B\wedge a + \widehat{B}\wedge \widehat{a}\right]\,.
    \label{eq:DW_Zn}
\end{equation}
Here we have used a continuum formulation of the Dijkgraaf-Witten (see Sec.~5 of \cite{Kapustin:2014gua}). 
%
Here $a$ and $\widehat{a}$ are dynamical compact $\ms U(1)$ 1-form gauge fields while $B$ and $\widehat{B}$ are 2-form background gauge fields corresponding to the global 1-form symmetry of the model.
%
This theory is shown to be equivalent to the more conventional $\mbb Z_n$ gauge formulation in \cite{Dijkgraaf:1989pz} by integrating over $\widehat{a}$.
%
For simplicity, if we set $B=\widehat{B}=0$, then integrating over $\widehat{a}$ imposes ${\rm{d}}a=0 \ \text{mod} \ 2\pi$ and $\oint a\in \frac{2\pi}{n}\mbb Z$.
%
Together these two conditions make $a$ a $\mbb Z_n$ gauge field.

Another convenient formulation of the Dijkgraaf-Witten theory is on an oriented simplicial manifold $M$ using the framework of simplicial calculus.
%
Then instead of $\ms U(1)$ gauge field, we let $\frac{2\pi}{n}a$ and $\frac{2\pi}{n}\widehat{a}$ be 1-cochains $C^{1}(M,\mbb Z_n)$. This mapping is informed by the fact that on-shell the holonomies of these fields are quantized to $\mbb Z_n\subset \ms{U}(1)$.
%
We choose this normalization such that on each 1-cell, $a$ and $\widehat{a}$ take values in $\left\{0,1,\dots,n\right\}$. Making these substitutions in \eqref{eq:DW_Zn}, one obtaines
\begin{equation}
    S=\frac{2\pi i}{n}\int\left\{\widehat{a}\cup {\rm d}a +{\rm p} a \cup \frac{\rm{d} a}{n} + \left[B\cup a+ \widehat{B}\cup \widehat{a}\right]\right\}\,.
\end{equation}
One can integrate out $\widehat{a}$ such that $a \in Z^{1}(M,\mbb Z_n)$. Upon doing so, it is more rigorous to understand ${\rm d}a/n$ as ${\rm{Bock}}(a)$.
%
The gauge invariant topological operators in the theory are
\begin{equation}
\begin{split}
    W_{(\rm{q,m})}(\gamma)=\exp\left\{\frac{2\pi i}{n}\oint_{\gamma}\rm{q}a+{\rm}\widehat{a}\right\}\,,
\end{split}
\end{equation}
where ${\rm{q}}\in \rm{Rep}(\mbb Z_n)\cong \mbb Z_n$ and ${\rm{m}}\in \mbb Z_n$.
%
The correlation functions of the topological line operator can be computed straightforwardly using standard methods \cite{Tiwari:2016zru, Putrov:2016qdo}.
%
For instance consider two 1-cycles $\gamma_{1}$ and $\gamma_2$ embedded in $M=S^3$ such that they form a Hopf-link. The correlation function of two line operators with support on $\gamma_1$ and $\gamma_2$ is
\begin{equation}
    \Big \langle W_{(\rm{q}_1,\rm{m}_1)}(\gamma_1) W_{(\rm{q}_2,\rm{m}_2)}(\gamma_2) \Big \rangle = \exp\left\{\frac{2\pi i}{n}(\rm{q}_1\rm{m}_2+\rm{q}_2\rm{m}_1)+\frac{4\pi i {\rm p}}{n^2}{\rm m_1m_2}\right\}\,.
\end{equation}

==> Appendices/BF_type_Z2_gauge_theory_Hamiltonians.tex <==
The toric code and double semion models refer to the fixed point limits of  deconfined phase of the $\mbb Z_{2}$ and twisted $\mbb Z_2$ gauge theory, where the twist is in the sense of Dijkgraaf-Witten theory \cite{Dijkgraaf:1989pz}.
%
The fixed point Hamiltonians have the form 
\begin{equation}
\begin{split}
    \mathcal H_{\rm{T.C}}&=-\sum_{\ms v}\prod_{\ms e \supset \ms v} \sigma^{z}_{\ms e} - \sum_{\triangle}\prod_{\ms e \subset \partial \triangle}\sigma^{x}_{\ms e}\,, \\
    \mathcal H_{\rm{D.S}}&=-\sum_{\ms v}\prod_{\ms e \supset \ms v} \sigma^{z}_{\ms e}\prod_{\ms e \in \partial {\rm{Hex}}_{\ms v}}i^{\frac{1-\sigma^{x}_{\ms e}}{2}}- \sum_{\triangle}\prod_{\ms e \subset \partial \triangle}\sigma^{x}_{\ms e}\,.
\label{eq:quantum doubles}
\end{split}
\end{equation}
Let us work in the eigen basis of $\sigma^{x}$ such that 
\begin{equation}
    \sigma^{x}_{\ms e}|a\rangle =(-1)^{a[\ms e]}|a\rangle\,, 
\end{equation}
where $a\in C^{1}(\Sigma_{\triangle},\mbb Z_2)$ and $a[\ms e]$ denotes the evaluation of $a$ on the edge $\ms e$. Therefore, we can straightforwardly write the operator in \eqref{eq:quantum doubles} defined on the  faces $\triangle$ as (see Fig.\ref{Fig:sigma_x in gauge basis})
\begin{equation}
    \prod_{\ms e \subset \partial \triangle}\sigma^{x}_{\ms e} = \sum_{a}\exp\left\{i\pi\oint_{\partial \triangle}a\right\}|a\rangle \langle a|
    \equiv
    \exp\left\{i\pi\oint_{\partial \triangle}\widehat{a}\right\}
    \,.
\end{equation}
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.8\textwidth]
{Figures_hand_drawn/Wilson.jpg}    
\end{center}
\caption{The operator $\sigma^{x}$ in the basis $\left\{|a\rangle\right\}$ is depicted by a blue line on the edge.}
\label{Fig:sigma_x in gauge basis}
\end{figure}

\medskip \noindent Similarly, the operators $\sigma^{z}_{\ms e}$ change the eigenvalue $a[\ms e]$ to $a[\ms e]+ 1 \ \rm{mod} \ 2$. We may describe this operator more generally via a cochain $b\in C^{1}(\Sigma^{\rm{dual}}_{\triangle},\mbb Z_2)$ on the dual lattice $\Sigma^{\rm{dual}}_{\triangle}$. This is possible when $\Sigma$ is two dimensional, since there is a bijection between the edges of the lattice and the dual lattice.
%
We will denote the dual cochains as green strings on the dual lattice (see Fig.~\ref{Fig:sigma_z in gauge basis})
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures_hand_drawn/tHooft.jpg}    
\end{center}
\caption{The operator $\sigma^{z}$ in the basis $\left\{|a\rangle\right\}$ is depicted by a green line on an edge $\ms e^{\vee}\subset \Sigma^{\rm{dual}}_{\triangle}$ which is dual to $\ms e \subset \Sigma_{\triangle}$.}
\label{Fig:sigma_z in gauge basis}
\end{figure}

\newl Then the Pauli algebra is represented as the string algebra {\AT{insert a tikz eqn depicting this}}.
%
With this reinterpretation of the operators acting on the edge Hilbert space, let us reinterpret the Hamiltonian.
%
It is easy to confirm that there is the following map of operators {\AT{add pictorial depiction of these operators}}
\begin{equation}
\begin{alignedat}{2}
    \prod_{\ms e \subset \partial\triangle} \sigma^{x}_{\ms e} 
    &\longleftrightarrow&& 
    \exp\left\{i\pi \oint_{\partial \triangle} \widehat{a}\right\}\,, \\ 
    \prod_{\ms e \supset \ms v} \sigma^{z}_{\ms e}     &\longleftrightarrow&& 
    \exp\left\{i\pi \oint_{\gamma^{\vee}_{\ms v}}\widehat{b}\right\}\,, \\
    \prod_{\ms e \supset \ms v} \sigma^{z}_{\ms e}\prod_{\ms e \in \partial {\rm{Hex}}_{\ms v}}i^{\frac{1-\sigma^{x}_{\ms e}}{2}}  
    &\longleftrightarrow&& 
    \exp\left\{i\pi \oint_{\gamma^{\vee}_{\ms v}}\widehat{b}+\frac{i\pi}{2}\oint_{\partial \rm{Hex}_{\ms v}}\widehat{\widetilde{a}} \right\}\,,
\end{alignedat}
\end{equation}
where $\gamma^{\vee}_{\ms v}$ is a smallest possible loop on the lattice $\Sigma_{\triangle}^{\rm{dual}}$ linking with the vertex $\ms v \subset \Sigma_{\triangle}$ and $\widehat{\widetilde{a}}$ is the operator corresponding to the $\mbb Z_4 $ lift of $a$.

\newl With this we can re-express the Hamiltonians in \eqref{eq:quantum doubles} as
\begin{equation}
\begin{split}
    \mc H_{\rm{T.C}}&= -  \sum_{\ms v} \exp\left\{i\pi \oint_{\gamma^{\vee}_{\ms v}}\widehat{b}\right\} - \sum_{\triangle}\exp\left\{i\pi \oint_{\partial \triangle} \widehat{a}\right\}\,, \\
   \mc H_{\rm{D.S}}&= -  \sum_{\ms v} \exp\left\{i\pi \oint_{\gamma^{\vee}_{\ms v}}\widehat{b}+\frac{i\pi}{2}\oint_{\partial \rm{Hex}_{\ms v}}\widehat{\widetilde{a}} \right\} - \sum_{\triangle}\exp\left\{i\pi \oint_{\partial \triangle} \widehat{a}\right\}\,,
   \label{eq:TC and DS in loop basis}
\end{split}
\end{equation}
It is useful to define the following line operators
\begin{equation}
    \mc W_{(\ms q, \ms m)}^{(p)}(L) := \exp\left\{
    i\pi \ms q\oint_{\gamma}\widehat{b}+\frac{i\pi p\ms q}{2}\oint_{\gamma^{\vee}}\widetilde{\widehat{a}}
    +i\pi \ms m\oint_{\gamma^{\vee}}\widehat{a}
    \right\}\,. 
    \label{eq:line_operators}
\end{equation}
Here $L=\left\{\gamma, \gamma^{\vee}\right\}$, i.e. a framed curve defined via a choice of two curves $\gamma$ and $\gamma^{\vee}$ on the direct and dual lattices respectively, see Fig \ref{Fig:Framed_line}.
%
In the definition \eqref{eq:line_operators}, $p=0$ and $p=1$ correspond to the topological line operators in the toric code and double semion models respectively.
%
The commutators of these line operators have the form 
\begin{equation}
\begin{split}
    \mc W_{(\ms q_1, \ms m_1)}^{(p)}(L_1)
    \mc W_{(\ms q_2, \ms m_2)}^{(p)}(L_2) 
    &=   \left[S^{(p)}_{(\ms q_1, \ms m_1);(\ms q_2, \ms m_2)} \right]^{{\rm{Int}} (L_1,L_2)}  \mc W_{(\ms q_2, \ms m_2)}^{(p)}(L_2)  \mc W_{(\ms q_1, \ms m_1)}^{(p)}(L_1)\,.    
\end{split}
\end{equation}
Where $S^{(p)}_{(\ms q_1, \ms m_1);(\ms q_2, \ms m_2)}$ is the S-matrix element in the toric code and double semion theories for $p=0,1$ respectively, which is
\begin{equation}
S^{(p)}_{(\ms q_1, \ms m_1);(\ms q_2, \ms m_2)}=\exp\left\{i\pi \left(\ms q_1\ms m_2+\ms q_2\ms m_1 + p \ms m_1\ms m_2\right) \right\}\,.    
\end{equation}
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.4\textwidth]{Figures_hand_drawn/Framed_wilson.jpg}    
\end{center}
\caption{A general dyonic line requires a choice of framing, i.e., a choice of a curve $\gamma$ on the direct lattice and another nearby curve $\gamma^{\vee}$ on the dual lattice.}
\label{Fig:Framed_line}
\end{figure}
It immediately follows that all closed line operator mutually commute for both choices of $p$.
%
Since the Hamiltonians \eqref{eq:TC and DS in loop basis} are constructed from loop operators, this immediately implies the exact solvability of these models.
%

\newl The low energy subspace of the two models can be distinguished by the topological properties of the line operators that commute with these models.
%
In particular by the statistics of the `flux' line operators labelled as $(0,1)$. We find
\begin{equation}
\begin{split}
    \mc W_{(0, 1)}^{(p)}(L_1)
    \mc W_{(0,1)}^{(p)}(L_2) 
    &=   (-1)^{p{\rm{Int}} (L_1,L_2)}  \mc W_{(0,1)}^{(p)}(L_2)  \mc W_{(0,1)}^{(p)}(L_1)\,.    
\end{split}
\end{equation}
\AT{Maybe add something about the mixed anomaly for the emergent 1fs?}

==> Appendices/Calculation_duality_of_characters.tex <==
In this appendix we detail the calculation of mapping of characters under gauging of $\mbb Z_2 \subset \mbb Z_4$, going from \eqref{eq:dual characters} to \eqref{eq:mapping of characters}. 
%
Firstly, inserting \eqref{eq:dual partition functions} into \eqref{eq:dual characters}, one gets
\begin{equation}
\begin{split}
    \chi_{\fr T^{\vee}}[q\,, \vec{\alpha}_{\ms n^{\vee}}\,,\alpha_{\ms k}\,,\ms n^{\vee}_t\,, \vec{\ms k}]&=\frac{1}{2^{2+N}}\sum_{\ms k_t,\vec{\ms n}^{\vee},\ms n_t.\vec{\ms n}}
    (-1)^{\alpha_{\ms k}\ms k_t+ \vec{\alpha}_{\ms n^{\vee}}\cdot \vec{\ms n}_{\vee}+ \ms n_{t}\ms n_{t}^{\vee}+ \vec{\ms n} \cdot\vec{\ms n}^{\vee} }\,.
\end{split}
\end{equation}

==> Appendices/generalizations_of_LevinGu.tex <==
The $\mbb Z_2$ symmetric Levin-Gu SPT model \cite{Levin:2012yb} is defined on a triangular lattice with each vertex $\ms v$ endowed with a two dimensional on-site Hilbert space $\mc V_{\ms v}\cong \mbb C^2$. 
%
There is a natural action of the Pauli operators on the local Hilbert space. The fixed point Hamiltonian has the form
    \begin{equation}
        H_{\rm{LG}}=-\sum_{j}\sigma^x_j\prod_{\triangle_{jj_1j_
2}}\exp\left\{\frac{2 \pi i}{8}(1-\sigma_{j_1}^z\sigma_{j_2}^z)\right\}\,. 
    \end{equation}
    For the purposes of generalization toi $\mbb Z_n$ SPTs, it is convenient to slightly re-formulate the Levin-Gu model. Let us denote the hexagon comprising of the six triangles that contain the vertex $j$ as ${\rm{Hex}}_j$. Next we denote the edges of the lattice as $\ms e$ and denote the source and target of each oriented edge as $\ms{s(e)}$ and $\ms{t(e)}$ respectively. An operator $\mc O_{\ms e}$ can be defined on the edge $\ms e$ which essentially  maps the $\left\{+1,-1\right\}$ eigenvalues of $\sigma^{z}_{\ms{t(e)}}\sigma^{z}_{\ms{s(e)}}$ to $\left\{0,1\right\}$. Such an operator has the form 
    \begin{equation}
        \mc O_{\ms e}= \sum_{\mu\in 0,1}\mu \frac{1+\mu \sigma^{z}_{\ms{s(e)}}\sigma^{z}_{\ms{t(e)}}}{2}= \sum_{\mu\in 0,1}\mu P_{\ms e}^{(\mu)}\,.
    \end{equation}
    Using these operators, the Levin-Gu model can be rewritten as
    \begin{equation}
        \mc{H}_{\rm LG}=
        -\sum_{j}\sigma^{x}_{j}\exp\left\{\frac{2\pi i}{4}\sum_{\ms e\in \partial {\rm{Hex}_j}} \mc O_{\ms e}\right\}
        = -\sum_{j}\sigma^{x}_j\exp\left\{i\pi \oint_{\partial 
         {\rm{Hex}_j}
        }{\rm{Bock}}(A)\right\}\,,
    \end{equation}
where in the final expression, we have introduced a $\mbb Z_2$ gauge field whose configuration on a link $\ms e$ is the eigenvalue of $\sigma^{z}_{\ms{t(e)}}\sigma^{z}_{\ms{s(e)}}$.

\medskip \noindent With this preparation, the generalization to $\mbb Z_n$symmetric SPTs is straightforward. 
%
Let us consider an oriented triangulation of a manifold $\Sigma$, with each vertex $\ms v$ of the triangulation endowed with a Hilbert space $\mc V_{\ms v}\simeq \mbb C_n$.
%
There is an action of the $\mbb Z_n$ clock and shift algebra given by 
\begin{equation}
    Z^{(n)}_{\ms v}   X^{(n)}_{\ms v'}=e^{2\pi i \delta_{\ms v \ms v'}/n }    X^{(n)}_{\ms v'}\, Z^{(n)}_{\ms v} 
    \label{eq:Zn_clock_algebra}
\end{equation}
Let the global $\mbb Z_n$ symmetry be generated by $\mc U= \prod_{\ms v}X^{(n)}_{\ms v}$. There are a total of $n$ SPTs labelled by $p\in \mbb Z_n$ with the fixed point Hamiltonians
    \begin{equation}
    \begin{split}
        \mc{H}^{(\mbb Z_n,p)}&=
        -\sum_{\ms v}X^{(n)}_{\ms v}\exp\left\{\frac{2\pi ip}{n^2}\sum_{\ms e\in \partial {\rm{Hex}_j}} \mc O^{(n)}_{\ms e}\right\}+ \text{H.c} \\
        &= -\sum_{j}X^{(n)}_{\ms v}\exp\left\{\frac{2\pi ip}{n}\oint_{\partial 
         {\rm{Hex}_{\ms v}}
        }{\rm{Bock}}(A)\right\}+ \text{H.c}\,,     
        \label{eq:Zn_Levin_Gu_generalization}
    \end{split}
    \end{equation}
    where we have defined 
    \begin{equation}
        \begin{split}
            \mc O^{(n)}_{\ms e}&= \sum_{\mu\in \mbb Z_n} \mu P_{\ms e}^{(n,\mu)}\,, \\
            P_{\ms e}^{(n,\mu)}&= \frac{1}{n}\sum_{\tau=0}^{n-1}e^{-\frac{2\pi i\tau \mu}{n}}(Z^{(n)}_{\ms s(\ms e)}\left(Z^{(n)}_{\ms t(\ms e)})^{\dagger}\right)^{\tau}\,. 
        \end{split}
    \end{equation}


==> Sections/1D_examples.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%
In this section, we describe the duality between $\mbb Z_4$ and $\mbb Z_2 \times \mbb Z_2$ symmetric (with a mixed anomaly) spin chains from the perspective of gauging subgroups described in generality in Sec.~\ref{Sec:gauging as topological dualities}.
%
The analysis is inspired by and closely follows Ref.~\cite{Zhang:2022wwn}. 
%
Let us consider a $\mbb Z_4$ spin chain defined on a lattice $\Lambda$. 
%
We will denote the collection of sites and links of this lattice as $\Lambda_0$ and $\Lambda_1$ respectively.
%
The Hilbert space of the model is $\mc V=\otimes_{j\in \Lambda_0 }\mc V_j $ where $\mc V_j\cong \mbb C^4$.
%
The local operator algebra is generated by two operators denoted as $S$ and $C$, where 
\begin{equation}
    S=
    \begin{pmatrix}
     0 & 0 & 0 & 1 \\
     1 & 0 & 0 & 0 \\
     0 & 1 & 0 & 0 \\
     0 & 0 & 1 & 0 \\ 
    \end{pmatrix}\,,
\quad 
    C=
    \begin{pmatrix}
     1 & 0 & 0 & 0 \\
     0 & i & 0 & 0 \\
     0 & 0 & -1 & 0 \\
     0 & 0 & 0 & -1 \\ 
    \end{pmatrix}\,.
\end{equation}
which satisfy $CS=iSC$, which is the $\mbb Z_4$ clock and shift algebra. We are interested in studying models with $\mbb Z_4$ symmetry which is generated by
\begin{equation}
    U^{(\mbb Z_4)}=\prod_{j}S_j\,.
\end{equation}
The bond algebra of such $\mbb Z_4$ symmetric spin chains is \cite{Cobanera:2009as, Cobanera_2011, Ortiz:2012zz}
\begin{equation}
    \mc B_{\Lambda}(\mbb Z_4)=\Big\langle C_jC_{j+1}^{\dagger}, S_j \Big| j\in \Lambda_0\Big \rangle\,, 
\end{equation}
i.e., any $\mbb Z_{4}$ symmetric operator acting on $\mc V$ is an element of $\mc B_{\Lambda}(\mbb Z_4)$.
%
Consider the $\mbb Z_4$ symmetric Hamiltonian
\begin{equation}
    \mc H_{\mbb Z_4}=-\sum_{j}\left[{\ms J_1}C_jC_{j+1}^{\dagger}
    +{\ms J_2}C^2_jC_{j+1}^{-2}
    +{\ms h_1}S_j
    +{\ms h_2}S^2_j
    +\rm{H.c}\right]\,,
    \label{eq:Z4_model}
\end{equation}
which can conveniently access all the gapped phases realized in $\mbb Z_4$ symmetric quantum systems in 1D by appropriately restricting the parameters $\left\{\ms{J}_1,\ms{J}_2, \ms{h}_1, \ms{h}_2\right\}$.
%
We may gauge the $\mbb Z_2$ subgroup of $\mbb Z_4$ by introducing $\mbb Z_2$ gauge degrees of freedom on the links $\Lambda_1$. 
%
Therefore the link Hilbert space is $\widetilde{\mc V}=\otimes_{j+1/2\in \Lambda_1}\widetilde{\mc V}_{j+1/2}$, where $\widetilde{\mc V}_{j+1/2}\cong \mbb C^2$. 
%
We will denote the Pauli operators acting on the link $j+1/2$ by $\tau^{\mu}_{j+1/2}$\footnote{To be consistent with \cite{Zhang:2022wwn}.} where $\mu=x,y,z$.
%
Next, we introduce the Gauss operator 
\begin{equation}
    \mc G_j=\tau^{z}_{j-1/2}S_j^2\tau^z_{j+1/2}\,,
\end{equation}
and require that the physical Hilbert space is invariant under the action of an arbitrary combination of Gauss operators 
\begin{equation}
    \mc G[\lambda]\equiv \prod_{j}\mc G_j^{\lambda_j}\,,
\end{equation}
where $\lambda \in C^0(\Lambda,\mbb Z_2)$.
%
The operator $\mc G[\lambda]$ acts via the following $\mbb Z_2$ gauge transformation
\begin{equation}
    \mc G[\lambda]:
    \begin{pmatrix}
        \tau^{x}_{\rm e} \\
        C^{\ms g}_{j}
    \end{pmatrix}
\longrightarrow
\begin{pmatrix}
    \tau^{x}_{\rm e}(-1)^{\rm d\lambda[\rm e]} \\
    C^{\ms g}_j (-1)^{\ms g \lambda_j}
\end{pmatrix}
\,,
\end{equation}
where $\ms g\in \mbb Z_4$. 
%
Next, we need to modify the Hamiltonian in eq.~\eqref{eq:Z4_model} by minimally coupling it to the gauge field $\tau^x_{j+1/2}$. 
%
Doing so, we get 
\begin{equation}
\begin{split}
       \mc H_{\mbb Z_4/\mbb Z_2}&=-\sum_{j}\left[{\ms J}_1C_j\tau^{x}_{j+1/2}C_{j+1}^{\dagger}
       +{\ms J_2}C_j^2C_{j+1}^{-2}
       +{\ms h_1}S_j
       +{\ms h_2}S_j^2
       +\rm{H.c}\right]\, \\
       &=-\sum_{j}\left[{\ms J}_1C_j\tau^{x}_{j+1/2}C_{j+1}^{\dagger}
       +{\ms J_2}C_j^2C_{j+1}^{-2}
       +{\ms h_1}S_j
       +{\ms h_2}\tau^{z}_{j-1/2}\tau^z_{j+1/2}\,
       +\rm{H.c}\right]\,,
       \label{eq:H_{Z4/Z2}}
\end{split}
\end{equation}
where in going to the second line, we have implemented the Gauss constraint on the terms proportional to $\ms h_2$.
%
What are the symmetries of the model $\mc H_{\mbb Z_4/\mbb Z_2}$? Firstly, it has the residual $\mbb Z_2$ symmetry generated by $U^{(\mbb Z_2)}=\prod_j S_j$. Note that on the physical (gauge invariant) Hilbert space, unlike $U^{(\mbb Z_4)}$, $U^{(\mbb Z_2)}$ generates a $\mbb Z_2$ symmetry since
\begin{equation}
    (U^{(\mbb Z_2)})^{2}=\prod_j S_j^2= \prod_j \mc G_j= 1\,. 
\end{equation}
There is another $\mbb Z_2$ symmetry in the gauged model, which is generated by 
\begin{equation}   V^{(\mbb Z_2)}=\prod_{j+1/2}\tau^{x}_{j+1/2}=\prod_{j+1/2}v_j\,, \quad v_j= C_j\tau^{x}_{j+1/2}C_{j+1}^{\dagger}\,.
\end{equation}
We emphasize that the local representative of $V^{(\mbb Z_2)}$ is $v_j$ and not the naive $\tau^x_{j+1/2}$, since the latter is not gauge invariant. 
%
Since the local representative of $V^{(\mbb Z_2)}$ and $U^{(\mbb Z_2)}$ do not commute, this precisely signals a mixed anomaly between the two $\mbb Z_2$ subgroups $\mbb Z_2^{U}$ and $\mbb Z_2^v$. 
%
See Ref.~\cite{Cheng:2022sgb} for a similar recent discussion on mixed anomalies of the $1+1d$ compact $\ms{U}(1)$ Boson theory formulated on the lattice as a modified Villain model (see also \cite{Sulejmanpasic:2019ytl, Fazza:2022fss}).

Next, we adapt the approach discussed in \cite{Zhang:2022wwn} and directly replace the $\mbb Z_4$ degrees of freedom on the vertices in the model \eqref{eq:Z4_model} by $\mbb Z_2\times \mbb Z_2$ degrees of freedom.
%
In analogy to the gauging procedure described above the first $\mbb Z_2$ corresponds to the gauge degrees of freedom on the links $\Lambda_1$. We will continue to denote the corresponding Pauli operators as $\tau^{\mu}_{j+1/2}$.
%
The second $\mbb Z_2$ corresponds to the residual $\mbb Z_2$ matter degrees of freedom that are left behind after gauging the $\mbb Z_2\subset \mbb Z_4$. 
%
We will denote the corresponding Pauli operators as $\sigma^{\mu}_{j}$.
%
A similar but more general  partial gauging construction appeared recently in Ref.~\cite{Delcamp:2023kew} in the context of analyzing global categorical symmetries in spin models.

Let us now describe how the various operators in the Hamiltonian in \eqref{eq:Z4_model} appear in the $\mbb Z_2\times \mbb Z_2$ basis, or equivalently how \eqref{eq:H_{Z4/Z2}} can be formulated in the $\mbb Z_2\times \mbb Z_2$ basis. 
\begin{itemize}
    \item We would like to implement $S_j$ which is the local representative of the symmetry $U^{(\mbb Z_2)}$ post gauging roughly as $\sigma^x_j$. However this isn't quite possible since the Gauss constraint implies that $S_j^2=\tau^z_{j-1/2}\tau^z_{j+1/2}$, therefore we impose\footnote{This operator was constructed in \cite{Zhang:2022wwn}. There is a seeming freedom in defining how $S_j$ maps to the $\mbb Z_2\times \mbb Z_2$ basis, i.e., if we only require that this operator squares to $\tau^{z}_{j-1/2}\tau^z_{j+1/2}$, then we can also define it, for example, as
\begin{equation}
        S_{j}\longleftrightarrow \sigma^{x}_j\left[P_{j-1,j}^{(+)}
        + P_{j-1,j}^{(-)}\tau^z_{j-1/2}
        \right]
\left[P_{j,j+1}^{(+)}
        + P_{j,j+1}^{(-)}\tau^{z}_{j+1/2}\right]\,,
    \end{equation}
but this should be fixed, once we $C_{j}C_{j+1}^{\dagger}$ by requiring the correct $\mbb Z_4$ clock-and-shift algebra.} 
    \begin{equation}
        S_{j}\longleftrightarrow \sigma^{x}_j\left[P_{j-1,j}^{(+)}
        + P_{j-1,j}^{(-)}\tau^z_{j-1/2}
        \right]
\left[P_{j,j+1}^{(+)}\tau^{z}_{j+1/2}
        + P_{j,j+1}^{(-)}\right]\,,
    \end{equation}
where $P^{(\epsilon)}_{i,j}:= \frac{1}{2}(1+ \epsilon \sigma^{z}_i\sigma^{z}_j)$. From which it follows that
\begin{equation}
    S_{j}^{\dagger}\longleftrightarrow \sigma^{x}_j\left[P_{j-1,j}^{(-)}
        + P_{j-1,j}^{(+)}\tau^z_{j-1/2}
        \right]
\left[P_{j,j+1}^{(-)}\tau^{z}_{j+1/2}
        + P_{j,j+1}^{(+)}\right]\,.
\end{equation}
It can easily be checked that the conditions $S_j^{2}=\tau^{z}_{j-1/2}\tau^{z}_{j+1/2}$ and $S_jS_j^{\dagger}=1$ are satisfied using $P^{(\epsilon)}_{j,j\pm 1}\sigma^{x}_{j}= \sigma^{x}_j P^{(\epsilon +1 \ \rm{mod} \ 2)}_{j,j\pm 1}$. The combination $S_j + S_j^{\dagger}$ which appears in the Hamiltonian, transforms as
\begin{equation}
    S_j+S_j^{\dagger}\longleftrightarrow \sigma^{x}_j \left\{
    (\tau_{j-1/2}^z+\tau_{j+1/2}^z)P_{j-1,j+1}^{(+)}+(1+\tau^{z}_{j-1/2}\tau^{z}_{j+1/2})P^{(-)}_{j-1,j+1}
    \right\}\,.
\end{equation}
In deriving this expression it is convenient to use the identity
\begin{equation}
    P_{j-1,j}^{(\epsilon_1)}P_{j,j+1}^{(\epsilon_2)}
    +
    P_{j-1,j}^{(\epsilon_1 +1 \ \rm{mod} \ 2)}P_{j,j+1}^{(\epsilon_2+1 \ \rm{mod} \ 2)}
    =
    P^{(\epsilon_1\epsilon_2)}_{j-1,j+1}\,.
\end{equation}

\item Next, we consider how the term $C_{j}C_{j+1}^{\dagger}$ maps to the ``dual'' $\mbb Z_2\times \mbb Z_2$ basis. There are two important requirements for the image of $C_{j}C_{j+1}^{\dagger}$---
it should have eigenvalues ${\rm{diag}}(1,i,-1,-i)$ and have the correct commutation relations with $S_j$. We find that the operator
\begin{equation}
    \tau^{x}_{j+1/2}\times i^{P^{(-)}_{j,j+1}}\,,
\end{equation}
satisfies these requirements. Let us again consider how the combination $C_{j}C_{j+1}^{\dagger}+\rm{H.c}$, which appears in the Hamiltonian \eqref{eq:Z4_model} transforms
\begin{equation}
    C_{j}C_{j+1}^{\dagger} + {\rm{H.c}}\longleftrightarrow 2 \tau^{x}_{j+1/2}P^{(+)}_{j,j+1}\,.
\end{equation}
\item The operator $C_j^{2}$ is then in the sign representation of the $\mbb Z_2$ global symmetry $U^{(\mbb Z_2)}$. We can replace $S_j\sim \sigma^x_j$. It can indeed be confirmed by simply taking the square of $\tau^{x}_{j+1/2}i^{P_{j,j+1}^{(-)}}$ that
    \begin{equation}
        C_{j}^{2}C_{j+1}^{-2}\longleftrightarrow \sigma_j^z\sigma^{z}_{j+1}\,.
    \end{equation}
\end{itemize}
Now we can finally write down the full model in the $\mbb Z_2\times \mbb Z_2$ basis
\begin{equation}
\begin{split}
     \widetilde{\mc H}_{\mbb Z_4/\mbb Z_2}&=-\sum_{j}\left[2{\ms J}_1\tau^{x}_{j+1/2}P_{j,j+1}^{(+)}
       +2{\ms J_2}\sigma^z_j\sigma^z_{j+1}
       +2{\ms h_2}\tau^{z}_{j-1/2}\tau^z_{j+1/2}\,.
       \right] \\    
       & - \sum_{j}\ms{h}_1 \sigma^{x}_j \left\{
    (\tau_{j-1/2}^z+\tau_{j+1/2}^z)P_{j-1,j+1}^{(+)}+(1+\tau^{z}_{j-1/2}\tau^{z}_{j+1/2})P^{(-)}_{j-1,j+1}
    \right\}\,.
    \label{eq:Z4/Z2 model in Z2Z2 basis}
\end{split}
\end{equation}
This model has a $\mbb Z_2\times \mbb Z_2$ symmetry generated by
\begin{equation}
    \begin{split}
        U^{(\mbb Z_2)}=\prod_{j}\sigma^{x}_j,\qquad V^{(\mbb Z_2)}=\prod_{j}\tau^{x}_{j+1/2}P^{(-)}_{j,j+1}\,.
    \end{split}
\end{equation}
Now we analyze and compare the gapped phases realized in the model \eqref{eq:Z4_model} with $\mbb Z_4$ symmetry with the model \eqref{eq:Z4/Z2 model in Z2Z2 basis} with $\mbb Z_2\times \mbb Z_2$ symmetry with a mixed anomaly. In general, it is known that the classification of gapped phases realized in 1+1d quantum system with $\ms G$ global symmetry and $\omega \in H^{3}(\ms G,\ms U(1))$ anomaly is given by the tuple $(\ms H,\psi)$ with $\ms H\subset \ms G $ such that $\omega|_{\ms H}$ is trivial in $H^{3}(\ms H,\ms U(1))$ and $\psi\in H^{2}(\ms H, \ms U(1))$.
%
Physically, the subgroup $\ms H$ corresponds to the subgroup of $\ms G$ preserved by the ground state in the given gapped phase, while $\psi$ realizes the topological nature of the symmetry realization, i.e., whether the ground state is an $\ms H$ SPT or not.
%
It follows that $\mbb Z_4$ symmetric systems realize three gapped phases labelled by the three possible subgroups of $\mbb Z_4$\footnote{Recall that $H^2(\mbb Z_4,\ms U(1))$ is trivial.}--- $\mbb Z_4,\mbb Z_2$ and $\mbb Z_1$.
%
Similarly, there are three gapped phases realized in $\mbb Z_2\times \mbb Z_2$ symmetric models with a mixed anomaly given by the representative cocycle
\begin{equation}
    \omega(\ms g,\ms h,\ms k)=\exp\left\{\frac{i \pi}{2} \ms g_1(\ms h_2+\ms k_2-[\ms h_2+\ms k_2]_2)\right\}\,,
\end{equation}
where $\ms g =(\ms g_1,\ms g_2)\in \mbb Z_2\times \mbb Z_2$ etc. and $[\ms h_2+\ms k_2]_2\equiv \ms h_2+\ms k_2 \ \rm{mod} \ 2$. The three gapped phases correspond to picking subgroups of $\mbb Z_2\times \mbb Z_2$ for which the cocycle is trivialized. There are two (non-diagonal) subgroups $\mbb Z_2\cong (\ms g_1,0)$ or $(0,\ms g_2)$ and a trivial subgroup $(\ms 0,\ms 0)\cong \mbb Z_1$ which give a total of three possibilities.
%
Atleast at the level of number of gapped phases seem to match.
%
Let us now describe in detail the correspondence between gapped phases in these two dual models:
\begin{itemize}
    \item Consider the $\mbb Z_4$ symmetric paramagnet in the model \eqref{eq:Z4_model}. This appears in the limit in parameter space where $\ms h_{1,2}$ are much larger than $\ms J_{1,2}$. On the gauged side, clearly, for large enough $\ms h_2$, the operator $\tau^{x}_{j+1/2}$ acquires a ground state expectation value which spontaneously breaks $V^{(\mbb Z_2)}$ symmetry. \AT{Need to show that $U^{\mbb Z_2}$ is preserved by the ground state.}
    \item Next, let us consider the partial symmetry broken phase in the model \eqref{eq:Z4_model}. This occurs when $\ms h_2$ and $\ms J_2$ are much larger than the other two parameters. Clearly the full $\mbb Z_2\times \mbb Z_2$ symmetry is broken in \eqref{eq:Z4/Z2 model in Z2Z2 basis}.
    \item Finally, consider the fully symmetry-broken phase fpr th parameter regime $\ms J_{i}\gg \ms h_i$. It can easily be checked correspondingly, in \eqref{eq:Z4/Z2 model in Z2Z2 basis}, the $U^{(\mbb Z_2)}$ symmetry is spontaneously broken since $\sigma^{z}_{j}$ acquires a ground state expectation value.
\end{itemize}
The above inferences can also be made on general grounds. Recall from Sec.~\ref{Sec:gauging as topological dualities} that the partition function of the partially gauged model model is given by 
\begin{equation}
    \mc Z_{\mbb Z_4/\mbb Z_2}[A^{(U)},A^{(V)}]=\frac{1}{2}\sum_{a\in H^{1}(M,\mbb Z_2)}\mc Z_{\mbb Z_4}[A^{(U)},a]\exp\left\{i\pi \int_{M} a\cup A^{(V)}\right\}\,,
    \label{eq:Z4 to Z4/Z2 duality in 1D}
\end{equation}
Now, in the fixed point limit, the partition functions for the $\mbb Z_4$ symmetric models are known to by 
\begin{equation}
\begin{alignedat}{2}
    \mc Z_{\mbb Z_4}[A^{(U)},A]&= 1 \quad &&(\rm{paramagnet})\,,  \\
    \mc Z_{\mbb Z_4}[A^{(U)},A]&= 2\delta_{A^{(U)},0} \quad &&(\rm{partial  \ symmetry \  broken})\,,  \\
    \mc Z_{\mbb Z_4}[A^{(U)},A]&= 4\delta_{A^{(U)},0}\delta_{A,0} \quad &&(\rm{fuly  \ symmetry \  broken})\,.
\end{alignedat}
\end{equation}
Inserting these topological partition functions into the formula for the dual partition function in \eqref{eq:Z4 to Z4/Z2 duality in 1D} one obtains
\begin{itemize}
    \item For the $\mbb Z_4$ paramagnet:
    \begin{equation}
        \mc Z_{\mbb Z_4/\mbb Z_2}[A^{(U)},A^{(V)}]=2\delta_{A^{V},0}\,,
    \end{equation}
    where we have used the formula (with $M=T^2$)
    \begin{equation}
        \frac{1}{|H^{1}(M,\mbb Z_2)|}\sum_{a\in H^{1}(M,\mbb Z_2)}\exp\left\{i\pi \int a\cup f(A)\right\}=\delta_{f(A),0}\,.
    \end{equation}
    This corresponds to spontaneous breaking of $V^{(\mbb Z_2)}$ in the partially gauged model.
    \item For the partial symmetry broken phase, we find
    \begin{equation}
    \begin{split}
    \mc Z_{\mbb Z_4/\mbb Z_2}[A^{(U)},A^{(V)}]&=\sum_{a}\delta_{A^{(U)},0}\exp\left\{i\pi \int_{M} a\cup A^{(V)}\right\}\\
    &= 4 \delta_{A^{(U)},0}\delta_{A^{(V)},0}\,,
    \end{split}
    \end{equation}
    which corresponds to the phase where the $\mbb Z_2\times \mbb Z_2$ is broken in the partially gauged theory.
    \item Similarly, it can be checked that the partition function of the partially gauged theory dual to the fully symmetry-broken model is
    \begin{equation}
        \mc Z_{\mbb Z_4/\mbb Z_2}[A^{(U)},A^{(V)}]=2\delta_{A^{(U)},0}\,.
    \end{equation}
    which corresponds to the phase where the $\mbb Z_2\times \mbb Z_2$ broken to the $\mbb Z_2^U$ subgroup.
\end{itemize}


